Herding Cats - Modelling, simulation, testing, and data-mining for weak memory

We propose an axiomatic generic framework for modelling weak memory. We show how to instantiate this framework for SC, TSO, C++ restricted to release-acquire atomics, and Power. For Power, we compare our model to a preceding operational model in which we found a flaw. To do so, we define an operational model that we show equivalent to our axiomatic model. We also propose a model for ARM. Our testing on this architecture revealed a behaviour later acknowledged as a bug by ARM, and more recently 33 additional anomalies. We offer a new simulation tool, called herd, which allows the user to specify the model of his choice in a concise way. Given a specification of a model, the tool becomes a simulator for that model. The tool relies on an axiomatic description; this choice allows us to outperform all previous simulation tools. Additionally, we confirm that verification time is vastly improved, in the case of bounded model-checking. Finally, we put our models in perspective, in the light of empirical data obtained by analysing the C and C++ code of a Debian Linux distribution. We present our new analysis tool, called mole, which explores a piece of code to find the weak memory idioms that it uses.

==> equiv.tex <==
\section{Equivalence of axiomatic model and intermediate machine (proof of \mylem\ref{lem:equiv})}
\label{sec:equiv}

We give here the details of the proof of equivalence of our axiomatic model,
described in~\mysec\ref{sec:model}, and our intermediate machine, given in
\mysec\ref{sec:pldi}. We first show one implication:
\begin{lemma}\label{lem:interm-ax}
All behaviours allowed by the intermediate machine are allowed by the axiomatic model.
\end{lemma}

then the other:
\begin{lemma}\label{lem:ax-interm}
All behaviours allowed by the axiomatic model are allowed by the intermediate machine.
\end{lemma}

\subsection{From intermediate machine to axiomatic model (proof of \mylem\ref{lem:interm-ax})}

We show here that a path of labels~$\textsf{p}$ relative to a set of
events~$\evts$ and a program order~$\po$ accepted by our intermediate machine
leads to a valid axiomatic execution. We show that the
execution~$(\evts,\po,\co(\evts,\textsf{p}),\rf(\evts,\textsf{p}))$ as defined
in \mysec\ref{sec:model} is valid in our axiomatic model.

\paragraph{Well formedness of $\co(\evts,\textsf{p})$ \!\!\!\!} follows from
\textsf{p} being a total order.

\paragraph{Well formedness of $\rf(\evts,\textsf{p})$ \!\!\!\!} follows
from the fact that we require that each read $r$ in $\evts$ has a unique
corresponding write $w$ in $\evts$, s.t. $r$ and $w$ have same address and
value, and $\Flush(w,r)$ is a label of \textsf{p}.

\paragraph{The \textsc{uniproc} axiom holds: \!\!\!\!} we show that
\textsf{CoWW}, \textsf{CoRW1}, \textsf{CoRW2}, \textsf{CoWR} and \textsf{CoRR}
are forbidden. \fixme{jade: CoRR?}

\paragraph{\textsf{CoWW} is forbidden: \!\!\!\!} suppose as a
contradiction two writes $e_1$ and $e_2$ to the same address s.t. $(e_1,e_2)
\in \po$ and $(e_2,e_1) \in \co(\evts,\textsf{p})$. The first hypothesis
entails that $(\Del(e_1),\Del(e_2)) \in \textsf{p}$. The second hypothesis
means by definition that $(\Del(e_2),\Del(e_1)) \in \textsf{p}$. This is a
contradiction of the acyclicity of \textsf{p}.
 
\paragraph{\textsf{CoRW1} is forbidden: \!\!\!\!} suppose as a
contradiction a read $r$ and a write $w$ relative to the same address, s.t.
$(r,w) \in \po$ and $(w,r) \in \rf(\evts,\textsf{p})$. Since \textsf{p} respects
$\po$ and is total, we know that $(\Del(w,r),\Del(w)) \in \textsf{p}$. Thus we have $r \in
\queue$ when we are about to take the transition $\Del(w)$: this contradicts
the \textsf{dw}$_2$ premiss of the \textsc{Write to buffer} transition. 

\paragraph{\textsf{CoRW2} is forbidden: \!\!\!\!} suppose as a
contradiction a read $r$ and two writes $w_1$ and $w_2$ relative to the same
address, s.t. $(r,w_2) \in \po$ and $(w_2,w_1) \in \co(\evts,\textsf{p})$ and
$(w_1,r) \in \rf(\evts,\textsf{p})$. Since $\textsf{p}$ respects $\po$ and is
total, we have $(\Del(w_1,r),\Del(w_2)) \in \textsf{p}$. Thus $w_1$ cannot be
visible to $r$ as it is $\co$-after $w_2$, $w_2$ itself being either equal or
$\co$-after the first write $w_a$ in $\poloc$ after $r$. This contradicts the
premiss $\textsf{dr}_1$ of the \textsc{Delay read} transition.

\paragraph{\textsf{CoWR} is forbidden: \!\!\!\!} suppose as a
contradiction two writes $w_0$ and $w_1$ and a read $r$ relative to the same
address, s.t. $(w_1,r) \in \po$, $(w_0,r) \in \rf(\evts,\textsf{p})$ and
$(w_0,w_1) \in \co(\evts,\textsf{p})$. Since $\textsf{p}$ respects $\po$ and is
total, we have $(\Del(w_1),\Del(w_0,r)) \in \textsf{p}$. Thus $w_0$ cannot be
visible to $r$ as it is $\co$-before $w_1$, $w_1$ being itself either equal or
$\co$-before the last write $w_b$ in $\poloc$ before $r$. This contradicts the
premiss $\textsf{dr}_1$ of the \textsc{Delay read} transition.

\paragraph{\textsf{CoRR} is forbidden: \!\!\!\!} suppose as a
contradiction a write $w$ and two reads $r_1$ and $r_2$ relative to the same
address, s.t. $(r_1,r_2) \in \po$, $(r_2,w) \in \fr$ and $(w,r_1) \in \rf$.
\fixme{TODO: decide what we do with CoRR}

\paragraph{The \textsc{thin air} axiom holds: \!\!\!\!} suppose as a
contradiction that there is a cycle in $\transc{\hb}$, \ie there is an event
$x$ s.t. $(x,x) \in \transc{(\mo{\transc{(\ppo \cup \fences)}} \cup
\mo{\rfe})}$. Thus there exists $y$ s.t. \textsf{(i)} $(x,y) \in \mo{(\ppo} \cup$
$\mo{\transc{\fences)}}; \mo{\rfe}$ and \textsf{(ii)} $(y,x) \in
\transc{(\mo{\transc{(\ppo \cup \fences)}}; \mo{\rfe})}$. Note that $x$ and $y$
are reads, since the target of $\rf$ is always a read.

We now show that \textsf{(iii)} for two reads $r_1$ and $r_2$, having
$(r_1,r_2) \in \transc{(\mo{\transc{(\ppo \cup \fences)}} \cup \mo{\rfe})}$
implies $(\Flush(r_1),\Flush(r_2)) \in \textsf{p}$ --- we are abusing our
notations once again here, writing $\Flush(r)$ instead of $\Flush(w,r)$ where
$w$ is the write from which $r$ reads. From the fact \textsf{(iii)} and the
hypotheses \textsf{(i)} and \textsf{(ii)}, we derive a cycle in $\textsf{p}$, a
contradiction since \textsf{p} is an order.

Proof of \textsf{(iii)}: let us show the base case; the inductive case follows
immediately. Let us have two reads $r_1$ and $r_2$ s.t. $(r_1,r_2) \in
\mo{\transc{(\ppo \cup \fences)}};\mo{\rfe})$. Thus there is $w_2$ s.t.
$(r_1,w_2) \in (\ppo \cup$ $\transc{\fences)}$ and $(w_2,r_2) \in \rfe$. Since
\textsf{p} is total, we have either the result or $(\Flush(w_2,r_2),\Flush(r_1))
\in \textsf{p}$.  Suppose the latter: thus when we are about to take the
\textsc{Read from pool} transition triggered by the label $\Flush(w_2,r_2)$, we
contradict the premiss $\textsf{df}_2$, because we have $(r_1,w) \in
\transc{(\ppo \cup \fences)}$ and $r_1$ still in the pool since $\Del(r_1)$
always precedes $\Flush(r_1)$, which is itself after the label $\Flush(r_2)$
that we are about to process.  

\paragraph{The \textsc{causality} axiom holds: \!\!\!\!} suppose as a
contradiction that the relation $\efr;\prop;\rstar{\hb}$ is not irreflexive,
\ie there are $w$ and $r$ s.t. $(r,w_2) \in \efr$ and $(w_2,r) \in
\prop;\rstar{\hb}$. Since $(r,w_2) \in \efr$, we have \textsf{(i)}
$(\Del(r),\Del(w_2)) \in \textsf{p}$. \fixme{jade: justify} Note that $(r,w_2)
\in \fr$ implies the existence of a write $w_1$ s.t. $(w_1,w_2) \in \co$ and
$(w_1,r) \in \rf$.

We now show that \textsf{(ii)} having $(w_1,w_2) \in \co$, $(w_1,r) \in \rf$
and $(w_2,r) \in \prop;\rstar{\hb}$ implies $(\Del(w_2),\Del(r))$ $\in
\textsf{p}$. From \textsf{(i)} and \textsf{(ii)}, we derive a cycle in
\textsf{p}, a contradiction since \textsf{p} is an order.

Proof of \textsf{(ii)}: let us have two writes $w_1, w_2$ and a read $r$
relative to the same address s.t.  $(w_1,w_2) \in \co$, $(w_1,r) \in \rf$ and
$(w_2,r) \in \prop;\rstar{\hb}$. Since \textsf{p} is total, we have either the
result or $(\Del(r),\Del(w_2))$ $\in \textsf{p}$. Suppose the latter: we
contradict the \textsf{dr}$_2$ hypothesis. Indeed when we are about to process
the transition triggered by the label $\Del(r)$, we have $(w_2,r) \in
\prop;\rstar{\hb}$ by hypothesis, and \textsf{(iii)} $(\Del(w_1),\Del(w_2)) \in
\textsf{p}$ (by definition of $(w_1,w_2) \in \co$). Thus we have $w_1$ already
in the buffer when we process $\Del(r)$, whereas $w_2$ is not in the buffer
yet. Hence $w_2$ will be placed after $w_1$ in buff when we process the
transition $\Del(w_2)$.

\paragraph{The \textsc{propagation} axiom holds: \!\!\!\!} suppose as a
contradiction that there is a cycle in $\transc{(\co \cup \prop)}$, \ie there
is an event $x$ s.t. $(x,x) \in \transc{(\co \cup \prop)}$. In other terms
there is $y$ s.t. \textsf{(i)} $(x,y) \in \co;\prop$ and \textsf{(ii)} $(y,x) \in \transc{(\co; \prop)}$.  
Note that $x$ and $y$ are writes, since the source of $\co$ is always a write.

We now show that \textsf{(iii)} for two writes $w_1$ and $w_2$, having
$(w_1,w_2) \in  \transc{(\co;\prop)}$ implies $(\Del(w_1),\Del(w_2)) \in \transc{\textsf{p}}$.
From the fact \textsf{(iii)} and the hypotheses \textsf{(i)} and \textsf{(ii)},
we derive a cycle in \textsf{p}, a contradiction since \textsf{p} is an order. 

Proof of \textsf{(iii)}:  let us show the base case; the inductive case follows
immediately. Let us have two writes $w_1$ and $w_2$ s.t. $(w_1,w_2) \in
\co;\prop$; thus there is a write $w$ s.t. $(w_1,w) \in \co$ and $(w,w_2) \in
\prop$. Since $\textsf{p}$ is total, we have either the result or
$(\Del(w_2),\Del(w_1)) \in \textsf{p}$. Suppose the latter: we contradict the
\textsf{dw}$_1$ hypothesis.  Indeed when we are about to take the \textsc{Write
to buffer} transition triggered by the label $\Del(w)$, we have $(w,w_2) \in
\prop$ by hypothesis, and $w_2$ already in the buffer: the hypothesis $(w_1,w)
\in \co$ means by definition that $(\Del(w_1),\Del(w)) \in \textsf{p}$, and we
also have $(\Del(w_2),\Del(w_1)) \in \textsf{p}$. Therefore when we are about
to process $\Del(w)$ we have placed $w_2$ in the buffer by taking the
transition $\Del(w_2)$.

\subsection{From axiomatic model to intermediate machine (proof of \mylem\ref{lem:ax-interm})}

We show here that an axiomatic execution $(\evts,\po,\co,\rf)$ leads to a valid
path $\textsf{p}$ of the intermediate machine. We build the path $\textsf{p}$
as described in \mysec\ref{sec:pldi}. Recall that we build \textsf{p} as the
linearisation of a certain relation \textsf{r} given in \mysec\ref{sec:pldi}.
We first need to show that we are allowed to linearise \textsf{r}, \ie that
\textsf{r} is acyclic. Then we show that none of the transitions of the machine
given in \myfig\ref{fig:mach} can block.

\paragraph{Linearisation of \textsf{r}: \!\!\!\!}

\paragraph{\textsc{Write to buffer} does not block: \!\!\!\!} suppose as a
contradiction a label $\Del(w)$ s.t. the transition of the intermediate machine
triggered by $\Del(w)$ blocks. This means that one of the premisses of the
\textsc{Write to buffer} rule is not satisfied. 

First case: the premiss \textsf{dw}$_1$ is not satisfied, \ie  there
exists $e$ in the buffer s.t. $(w,e) \in \prop$. Since $e$ is in the buffer
when we are about to process the label $\Del(w)$, we have \textsf{(i)} $(\Del(e),\Del(w))
\in \textsf{p}$. Since $(w,e) \in \prop$, we have \textsf{(ii)}
$(\Del(w),\Del(e)) \in \textsf{p}$ (recall from \mysec\ref{sec:pldi} that we
build \textsf{p} inductively; in particular the order of the $\Del(w)$
transitions in \textsf{p} respects the order of the corresponding events in
$\prop$).  From \textsf{(i)} and \textsf{(ii)}, we derive a cycle in
\textsf{p}, a contradiction since \textsf{p} is an order (since we build it as
a linearisation of a relation). 

Second case: the premiss \textsf{dw}$_2$ is not satisfied, \ie  there exists
$r$ in the pool s.t. $(r,w) \in \poloc$. Since $(r,w) \in \poloc$ we have
$(r,w) \in \ifr$; hence $(r,w) \in \ppo$. Thus we have \textsf{(i)}
$(\Flush(r),\Del(w)) \in \textsf{p}$. Moreover if $r$ is in the pool when we
are about to process $\Del(w)$, then $r$ is going to be flushed after writing
$w$ in the buffer, \ie \textsf{(ii)} $(\Del(w),\Flush(r)) \in \textsf{p}$. From
\textsf{(i)} and \textsf{(ii)}, we derive a cycle in \textsf{p}, a
contradiction since \textsf{p} is an order (since we build it as a
linearisation of a relation). \fixme{jade: make it clearer how we use the fact
that p comes from a valid axiomatic execution: which axiom do we contradict?} 

\paragraph{\textsc{Delay read} does not block: \!\!\!\!} suppose as a
contradiction a label $\Del(w,r)$ s.t. the transition of the intermediate
machine triggered by $\Del(w,r)$ blocks. This means that one of the premisses
of the \textsc{Delay read} rule is not satisfied. Note that since
$\Del(w,r)$ is a label of \textsf{p}, we have \textsf{(i)} $(w,r) \in \rf$. 

First case: the premiss~\textsf{dr}$_1$ is not satisfied, \ie $w$ is not
visible to~$r$. This contradicts the \textsc{uniproc} axiom. \fixme{jade: to
make better: how does visible in machine world implies visible in ax world?}  

Second case: the premiss~\textsf{dr}$_2$ is not satisfied, \ie there is a
write~$e$ s.t. $(w,e) \in \buff$ and $(e,r) \in \prop;\rstar{\hb}$.  Since
$(w,e) \in \buff$, by \textsf{(i)} we have $(w,e) \in \co$, thus $(r,e) \in
\fr$. Therefore we contradict the \textsc{causality} axiom. \fixme{jade: to
make better: how does buff implies co? how does prop;hb in machine world
implies prop;hb in ax world?}

\paragraph{\textsc{Read from pool} does not block: \!\!\!\!} suppose as a
contradiction a label $\Flush(w,r)$ s.t. the transition of the intermediate
machine triggered by $\Flush(w,r)$ blocks. This means that one of the premisses
of the \textsc{Read from pool} rule is not satisfied. 
%Note that since $\Flush(w,r)$ is a label of \textsf{p}, we have \textsf{(i)}
%$(w,r) \in \rf$.

First case: the premiss $\textsf{fr}_1$ is not satisfied, \ie $r$ is not in the
pool. This is impossible since we impose $(\Del(r),\Flush(r)) \in \textsf{p}$
when building \textsf{p} (\cf~\mysec\ref{sec:pldi}).

Second case: the premiss $\textsf{fr}_2$ is not satisfied, \ie there is a read
$e$ in the pool s.t. $(e,w) \in \transc{(\ppo \cup \fences)}$. We build
\textsf{p} s.t. \textsf{(i)} $(\Flush(e),\Del(w)) \in \textsf{p}$.  Moreover
since $e$ is in the pool when we are about to process $\Flush(r)$, we have
\textsf{(ii)} $(\Flush(r),\Flush(e)) \in \textsf{p}$. Finally, since
$\Flush(w,r)$ is a label of \textsf{p}, we have $(w,r) \in \rf$. Thus
$(\Del(w),\Del(r)) \in \textsf{p}$, which implies \textsf{(iii)}
$(\Del(w),\Flush(r)) \in \textsf{p}$. Indeed a \textsc{delay read} transition always
precedes the corresponding \textsc{read from pool} transition, \ie
$(\Del(r),\Flush(r) \in \textsf{p})$. From \textsf{(i)}, \textsf{(ii)} and
\textsf{(iii)} we derive a cycle in \textsf{p}, a contradiction. \fixme{jade:
make it clearer how we use the fact that p comes from a valid axiomatic
execution: which axiom do we contradict?}  


==> software.tex <==
\section{Towards software and distributed models\label{software}}


==> soundness.tex <==
\section{Soundness of axiomatic model \wrt PLDI machine (proof of \mythm\ref{thm:soundness})}
\label{sec:soundness}

We show here that a valid path of the PLDI machine leads to a valid path of our
intermediate machine. 

Formally, we assume given a path~\textsf{p} over a set of labels~$\mathbb{L}$.
We suppose that \textsf{(mns)} for any label~$l$ of~$\mathbb{L}$, there are a
number of steps~$n$, and three states~$s_0, s_1$ and~$s_2$ s.t. the PLDI
machine goes from~$s_0$ to~$s_1$ in~$n$ steps, following the path~\textsf{p} up
to~$l$ not included, then does one transition triggered by~$l$ from~$s_1$
to~$s_2$. 

We write $\ltopl(l)$ for the mapping from intermediate labels to PLDI labels,
\ie a \textsc{delay write} transition in the intermediate machine corresponds
to a commit write in the PLDI machinel; a \textsc{delay read} corresponds to a
satisfy read; a \textsc{read from pool} corresponds to a commit read.

We derive from this mapping the set $\mathbb{L}_i$ of intermediate labels that
we are concerned with, \ie $\dfn{\mathbb{L}_i}{\{l \mid \ltopl(l) \in
\mathbb{L}\}}$, and the corresponding intermediate path $\textsf{p}_i$, \ie
$\dfn{\textsf{p}_i}{\{(l_1,l_2) \mid (\ltopl(l_1),\ltopl(l_2)) \in
\textsf{p}\}}$.

We derive intermediate states from PLDI states as described in
\mysec\ref{sec:pldi}. 

We show that the property \textsf{(mns)} holds for the intermediate machine:
for any label~$l_i$ of~$\mathbb{L}_i$, there are a number of steps~$m$, and
three states~$\pstos(s_0), \pstos(s_1)$ and~$\pstos(s_2)$ s.t. the intermediate
machine goes from~$\pstos(s_0)$ to~$\pstos(s_1)$ in~$m$ steps, following the
path~$\textsf{p}_i$ up to~$l_i$ not included, then does one transition
triggered by~$l_i$ from~$\pstos(s_1)$ to~$\pstos(s_2)$. 

\fixme{TODO HERE state the two corresponding lemmas and refer to them in the
subsections' titles below}

Let $l_i$ be a label of~$\mathbb{L}_i$; by definition we know that there is a
PLDI label $l \in \mathbb{L}$ s.t. \textsf{(mns)} holds for the PLDI machine.
We take $n, s_0, s_1$ and $s_2$ as given by \textsf{(mns)}.

Since there are less possible intermediate labels than PLDI labels, the mapping
from intermediate to PLDI labels can only make the number of labels decrease.
In other terms, the intermediate path $\textsf{p}_i$ has a number of labels $m$
which is less than or equal to $n$. 

\subsection{A PLDI transition gives an intermediate transition}
We show here that if the PLDI machine can make a step from $s_1$ to $s_2$
triggered by $l$, then the intermediate machine can make a step from
$\pstos(s_1)$ to $\pstos(s_2)$ triggered by $l_i$.  We proceed by case
disjunction over the PLDI transition, and list below the three cases, under the
form \emph{``PLDI transition is intermediate transition''}.

\paragraph{Commit write is delay write:  \!\!\!\!\!\!} in the PLDI machine,
a commit write transition records this write as seen and makes this
write~$\co$-after all the writes to the same address that have been propagated
to its thread, which modifies our intermediate state adequately.

The PLDI transition guarantees that~$w$ had not been seen in~$s_1$. Now,
contradict the premiss~\textsf{dw}$_1$, \ie take a write~$e$ in~$\buff$
s.t.~$(w,e) \in \prop$. In that case, $(w,e) \in \prop$ guarantees that~$w$ was
propagated to the thread of~$e$ in~$s_1$. Therefore (\cf~\cite{ssa11}[p.~6,
premiss of \S~Propagate write to another thread], $w$ was seen in~$s_1$.

Now, contradict \textsf{dw}$_2$, \ie take a read $r$ in the pool s.t.~$(r,w)
\in \poloc$. We just committed~$w$, and commit order respects~$\poloc$
(\cf~\cite{ssa11}[p.~7, item 4 of \S~Commit in-flight instruction]), hence~$r$
is commited in~$s_2$, which contradicts its being in the pool.

\paragraph{Satisfy read is delay read: \!\!\!\!\!\!} in the PLDI machine, a
satisfy read transition does not modify the state (\ie $s_1=s_2$). The
intermediate state gets adequately modified however: the buffer remains the
same, but we augment the pool with the read that got satisfied.

The PLDI transition guarantees that $w$ is visible to $r$ (since the PLDI
machine prevents~\textsf{CoWR} and~\textsf{CoRW2}), ensuring~\textsf{dr$_1$}
premiss. It also guarantees that $w$ is the latest write to~$\loc(r)$
propagated the thread of~$r$; hence there is no write~$e$ in the buffer
after~$w$ s.t.~$(e,r) \in \prop;\rstar{\hb}$.  \fixme{jade: etre plus explicite
sur pourquoi c'est le cas ici} This ensures the~\textsf{dr$_2$} premiss.

\paragraph{Commit read is read from pool: \!\!\!\!\!\!} in the PLDI machine,
a commit read transition does not modify the state. In the intermediate state,
the buffer remains the same, but we erase the read from the pool. \fixme{jade:
be clearer that this is by dfn of the pool}

Now, contradict the premiss~\textsf{df}$_2$, \ie take a read~$e$ in the pool
s.t.~$(e,w) \in \transc{(\ppo \cup \fences)}$. The fact that~$e$ is in the pool
means that~$e$ has not been committed yet. Yet, $r$ was satisfied by~$w$, which
means that~$w$ has been committed. Since commit order respects~$\transc{(\ppo
\cup \fences)}$ (\cf~\cite{ssa11}[p.~7, items 2, 3, 5, 6, 7 of \S~Commit
in-flight instruction]), hence~$e$ is committed in~$s_2$, a contradiction.

\subsection{A PLDI path gives an intermediate path}

We show here that if we have a PLDI path of length $n \neq 0$ from $s_0$ to $s_1$
following the path \textsf{p}, then we can derive an intermediate path of a
certain length $m$ from $\pstos(s_0)$ to $\pstos(s_1)$ following $\textsf{p}_i$
as defined above.

We proceed by induction over the length of $\textsf{p}_i$. If this length is
$0$, this means that \textsf{p} was exclusively composed of PLDI labels which
have no corresponding intermediate labels, in which case $\pstos(s_0) =
\pstos(s_1)$ and we have our result.

Otherwise, there exists an intermediate label $l'_i$ (possibly the \textsf{eof}
label marking the beginning of a path) which is the first intermediate label
before the last intermediate label $l_i$ of $\textsf{p}_i$. By definition of
$\textsf{p}_i$, we have $(\ltopl(l'_i),\ltopl(l_i)) \in \textsf{p}$.

We show that \textsf{(i)} there exists a PLDI state $s$ s.t. the PLDI machine goes from
$s_0$ to $s$ following \textsf{p} up to $\ltopl(l'_i)$ not included, then from
$s$ to $s_1$ following \textsf{p} up to $\ltopl(l_i)$ not included.

Since $l'_i$ is the first label before $l_i$, we know that there is no other
corresponding PLDI label between $\ltopl(l'_i)$ and $\ltopl(l_i)$ in
\textsf{p}. Therefore when the PLDI machine follows \textsf{p} from $s$ to
$s_1$ up to $\ltopl(l_i)$ not included, the intermediate machine only processes
one transition, which is triggered by $l_i$. 

Therefore we take this intermediate transition from $\pstos(s)$ to
$\pstos(s_1)$, and the inductive hypothesis gives us the intermediate path from
$\pstos(s_0)$ to $\pstos(s)$.


==> verif.tex <==
\section{Verification\label{sec:verif}}

